Toward Wheeled Mobility on Vertically Challenging Terrain: Platforms, Datasets, and Algorithms

Most conventional wheeled robots can only move in flat environments and simply divide their planar workspaces into free spaces and obstacles. Deeming obstacles as non-traversable significantly limits wheeled robots' mobility in real-world, extremely rugged, off-road environments, where part of the terrain (e.g., irregular boulders and fallen trees) will be treated as non-traversable obstacles. To improve wheeled mobility in those environments with vertically challenging terrain, we present two wheeled platforms with little hardware modification compared to conventional wheeled robots; we collect datasets of our wheeled robots crawling over previously non-traversable, vertically challenging terrain to facilitate data-driven mobility; we also present algorithms and their experimental results to show that conventional wheeled robots have previously unrealized potential of moving through vertically challenging terrain. We make our platforms, datasets, and algorithms publicly available to facilitate future research on wheeled mobility.

==> content/approach.tex <==
\section{APPROACH}
\label{sec::approach}
To improve upon existing navigation systems, the problem considered here is that of \emph{determining a parameter-selection strategy that allows a robot to move quickly and smoothly to its goal}.

We approach this problem as one of learning from human demonstration.
Namely, we assume that a human can provide a teleoperated demonstration of desirable navigation behavior in the deployment environment and we seek to find a set of planner parameters that can provide a good approximation of this behavior.
As we will show in Section \ref{sec::experiments}, when faced with a complex environment, a human demonstrator naturally drives differently in each regions of the environment such that no single set of planner parameters can closely approximate the demonstration in all states.
To overcome this problem, the human demonstration is divided into pieces that include consistent sensory observations and navigation commands. 
By segmenting the demonstration in this way, each piece---which we call a \emph{context}---corresponds to a relatively cohesive navigation behavior.
Therefore, it becomes more feasible to find a single set of planner parameters that imitates the demonstration well for each context.
% In the following, we formalize the problem definition and present the proposed method in stages.

\subsection{Problem Definition}
We assume we are given a robot with an existing navigation planner $G: \mathcal{X} \times \Theta \rightarrow \mathcal{A}$.
Here, $\mathcal{X}$ is the state space of the planner (e.g., current robot position, sensory inputs, navigation goal, etc.), $\Theta$ is the space of free parameters for $G$ (e.g., sampling density, maximum velocity, etc.), and $\mathcal{A}$ is the planner's action space (e.g., linear and angular velocity). 
Using $G$ and a particular set of parameters $\theta$, the robot performs navigation by repeatedly estimating its state $x$ and applying action $a = G(x;\theta)= G_{\theta}(x)$.
Importantly, we treat $G$ as a black-box, e.g., we do not assume that it is differentiable, and we need not even understand what each component of $\theta$ does.
%
In addition, a human demonstration of successful navigation is recorded as time series data $\mathcal{D} = \{ x^D_i, a^D_i, t^D_i \}_{i=1}^N$, where $N$ is the length of the series, and $x^D_i$ and $a^D_i$ represent the robot state and demonstrated action at time $t^D_i$.
%
Given $G$ and $\mathcal{D}$, the particular problem we consider is that of finding two functions: \textbf{(1)} a mapping $M: \mathcal{C} \rightarrow \Theta$ that determines planner parameters for a given {\em context} $c$, and \textbf{(2)} a parameterized context predictor $B_\phi: \mathcal{X} \rightarrow \mathcal{C}$ that predicts the context given the current state.
Given $M$ and $B_\phi$, our system then performs navigation by selecting actions according to $G(x; M(B_\phi(x)))$.
Note that since the formulation presented here involves only changing the {\em parameters} of $G$, the learned navigation strategy will still possess the benefits that many existing navigation systems can provide, such as assurance of safety.

\subsection{Demonstration Segmentation}
Provided with a demonstration, the first step of the proposed approach is to segment the demonstration into pieces---each of which corresponds to a single context only---so that further learning can be applied for each specific context.
This general segmentation problem can be, in principle, solved by any changepoint detection method~\cite{aminikhanghahi2017survey}.
Given $\mathcal{D}$, a changepoint detection algorithm $A_{\text{segment}}$ is applied to automatically detect how many changepoints exist and where those changepoints are within the demonstration.
Denote the number of changepoints found by $A_{\text{segment}}$ as $K-1$ and the changepoints as $\tau_1, \tau_2, \dots, \tau_{K-1}$ with $\tau_0 = 0$ and $\tau_K = N+1$, the demonstration $\mathcal{D}$ is then segmented into $K$ pieces $\{\mathcal{D}_k=\{x^D_i, a^D_i, t^D_i \,|\, \tau_{k-1} \leq i < \tau_k\}\}_{k=1}^K$.

\subsection{Parameter Learning} Following demonstration segmentation, we then seek to learn a suitable set of parameters $\theta^*_k$ for each segment $\mathcal{D}_k = \{x^D_i, a^D_i, t^D_i \,|\, \tau_{k-1} \leq i < \tau_k\}$.
To find this $\theta^*_k$, we employ {\em behavioral cloning} (\textsc{BC})~\cite{pomerleau1989alvinn}, i.e., we seek to minimize the difference between the demonstrated actions and the actions that $G_{\theta_k}$ would produce on $\{x^D_i\}$.
More specifically,
\begin{equation}
    \begin{split}
    \theta^*_k &= \argmin_{\theta} \sum_{(x, a) \in \mathcal{D}_k} ||a - G_{\theta}(x))||_H,
    \end{split}
    \label{eqn:bc}
\end{equation}
where $||v||_H = v^THv$ is the induced norm by a diagonal matrix $H$ with positive real entries, which is used for weighting each dimension of the action. A black-box optimization method $A_{\text{black-box}}$ is then applied to solve Equation \ref{eqn:bc}. Having found each $\theta^*_k$, the mapping $M$ is simply $M(k) = \theta^*_k$.

\subsection{Online Context Prediction}
At this point, we have a library of learned parameters and the mapping $M$ that is responsible for mapping a specific context to its corresponding parameters. All that remains is a scheme to dynamically infer which context the robot is in during \emph{execution}. To do so, we form a supervised dataset $\{x^D_i, c_i\}_{i=1}^N$, where $c_i = k$ if $x^D_i \in \mathcal{D}_k$. Then, a parameterized function $f_\phi(x)$ is learned via supervised learning to classify which segment $x^D_i$ comes from, i.e., 
\begin{equation}
    \phi^* = \argmax_\phi \sum_{i=1}^N \log \frac{\exp\big(f_\phi(x^D_i)[c_i]\big)}{\sum_{c=1}^K \exp{\big(f_\phi(x^D_i)[c]\big)}}.
\end{equation}
Given $f_\phi$, we define our context predictor $B$ according to
% \begin{equation}
%     B_\phi(x_t) = \argmax_c \sum_{i = t-p+1}^t \mathbbm{1}\big[(\argmax_{c'} f_\phi(x_i)[c']) = c\big].
%     \label{eqn:mode_switching}
% \end{equation}
\begin{equation}
    B_\phi(x_t) = \mode \Big\{\argmax_{c} f_\phi(x_i)[c],\,\, t-p < i \leq t \Big\}.
    \label{eqn:mode_switching}
\end{equation}
In other words, $B_\phi$ acts as a mode filter on the context predicted by $f_\phi$ over a sliding window of length $p$.

\begin{algorithm}[t]
\small
\caption{\textsc{appld}} \label{alg:appld}
\begin{algorithmic}[1]
    \STATE{// Training}
    \STATE{\textbf{Input:} the demonstration $\mathcal{D} = \{ x^D_i, a^D_i, t^D_i \}_{i=1}^N$, space of possible parameters $\Theta$, and the navigation stack $G$}.
    \STATE Call $A_{\text{segment}}$ on $\mathcal{D}$ to detect changepoints $\tau_1, \dots, \tau_{K-1}$ with $\tau_0=0$ and $\tau_K=N+1$.
    \STATE Segment $D$ into $\{\mathcal{D}_k=\{x^D_i, a^D_i, t^D_i \,|\, \tau_{k-1} \leq i < \tau_k\}\}_{k=1}^K$.
    \STATE Train a classifier $f_\phi$ on $\{x^D_i, c_i\}_{i=1}^N$, where $c_i = k$ if $x^D_i \in \mathcal{D}_k$.
    \FOR{$k=1:K$}
        \STATE Call $A_{\text{black-box}}$ with objective defined in Equation \ref{eqn:bc} on $\mathcal{D}_k$ to find parameters $\theta^*_k$ for context $k$.
    \ENDFOR
    \STATE Form the map $M(k) = \theta^*_k$, $\forall 1\leq k\leq K$.
    \STATE 
    \STATE{// Deployment}
    \STATE \textbf{Input:} the navigation stack $G$, the mapping $M$ from context to parameters, and the context predictor $B_\phi$.
    \FOR{$t=1:T$}
        \STATE Identify the context $c_t = B_\phi(x_t)$ according to Equation \ref{eqn:mode_switching}.
        \STATE Navigate with $G(x_t; M(c_t))$.
    \ENDFOR
\end{algorithmic}
\end{algorithm}

Taken together, the above steps constitute our proposed \textsc{appld} approach. During training, the above three stages are applied sequentially to learn a library of parameters $\{\theta^*_k\}_{k=1}^K$ (hence the mapping $M$) and a context predictor $B_\phi$. During execution, Equation \ref{eqn:mode_switching} is applied online to pick the right set of parameters for navigation. Algorithm \ref{alg:appld} summarizes the entire pipeline from offline training to online execution.

